Weighted Cheeger and Buser Inequalities, with Applications to Clustering and Cutting Probability Densities

In this paper, we show how sparse or isoperimetric cuts of a probability density function relate to Cheeger cuts of its principal eigenfunction, for appropriate definitions of `sparse cut' and `principal eigenfunction'. We construct these appropriate definitions of sparse cut and principal eigenfunction in the probability density setting. Then, we prove Cheeger and Buser type inequalities similar to those for the normalized graph Laplacian of Alon-Milman. We demonstrate that no such inequalities hold for most prior definitions of sparse cut and principal eigenfunction. We apply this result to generate novel algorithms for cutting probability densities and clustering data, including a principled variant of spectral clustering.

==> _ <==
@incollection{w17,
  title={Linear Elliptic Partial Differential Equations},
  author={Whiteley, Jonathan},
  booktitle={Finite Element Methods},
  pages={119--141},
  year={2017},
  publisher={Springer}
}
@article{SPIELMAN2007284,
title = "Spectral partitioning works: Planar graphs and finite element meshes",
journal = "Linear Algebra and its Applications",
volume = "421",
number = "2",
pages = "284 - 305",
year = "2007",
note = "Special Issue in honor of Miroslav Fiedler",
issn = "0024-3795",
doi = "https://doi.org/10.1016/j.laa.2006.07.020",
url = "http://www.sciencedirect.com/science/article/pii/S0024379506003454",
author = "Daniel A. Spielman and Shang-Hua Teng",
keywords = "Spectral methods, Spectral analysis, Graph partitioning, Eigenvalue problems, Graph embedding",
abstract = "Spectral partitioning methods use the Fiedler vectorâthe eigenvector of the second-smallest eigenvalue of the Laplacian matrixâto find a small separator of a graph. These methods are important components of many scientific numerical algorithms and have been demonstrated by experiment to work extremely well. In this paper, we show that spectral partitioning methods work well on bounded-degree planar graphs and finite element meshesâthe classes of graphs to which they are usually applied. While naive spectral bisection does not necessarily work, we prove that spectral partitioning techniques can be used to produce separators whose ratio of vertices removed to edges cut is O(n) for bounded-degree planar graphs and two-dimensional meshes and O(n1/d) for well-shaped d-dimensional meshes. The heart of our analysis is an upper bound on the second-smallest eigenvalues of the Laplacian matrices of these graphs: we prove a bound of O(1/n) for bounded-degree planar graphs and O(1/n2/d) for well-shaped d-dimensional meshes."
}

@inproceedings{SpielmanTeng2004,
 author = {Spielman, Daniel A. and Teng, Shang-Hua},
 title = {Nearly-linear Time Algorithms for Graph Partitioning, Graph Sparsification, and Solving Linear Systems},
 booktitle = {Proceedings of the Thirty-sixth Annual ACM Symposium on Theory of Computing},
 series = {STOC '04},
 year = {2004},
 isbn = {1-58113-852-0},
 location = {Chicago, IL, USA},
 pages = {81--90},
 numpages = {10},
 url = {http://doi.acm.org/10.1145/1007352.1007372},
 doi = {10.1145/1007352.1007372},
 acmid = {1007372},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {graph partitioning, graph sparsification, preconditioners},
} 

@inproceedings{Orecchia08,
  title={On partitioning graphs via single commodity flows},
  author={Orecchia, Lorenzo and Schulman, Leonard J and Vazirani, Umesh V and Vishnoi, Nisheeth K},
  booktitle={Proceedings of the fortieth annual ACM symposium on Theory of computing},
  pages={461--470},
  series={STOC '08},
  year={2008},
  organization={ACM}
}

@inproceedings{Orecchia2011,
 author = {Orecchia, Lorenzo and Vishnoi, Nisheeth K.},
 title = {Towards an SDP-based Approach to Spectral Methods: A Nearly-linear-time Algorithm for Graph Partitioning and Decomposition},
 booktitle = {Proceedings of the Twenty-second Annual ACM-SIAM Symposium on Discrete Algorithms},
 series = {SODA '11},
 year = {2011},
 location = {San Francisco, California},
 pages = {532--545},
 numpages = {14},
 url = {http://dl.acm.org/citation.cfm?id=2133036.2133078},
 acmid = {2133078},
 publisher = {Society for Industrial and Applied Mathematics},
 address = {Philadelphia, PA, USA},
} 
@inproceedings{sw18,
  author    = {Christian Sohler and
               David P. Woodruff},
  title     = {Strong Coresets for k-Median and Subspace Approximation: Goodbye Dimension},
  booktitle = {59th {IEEE} Annual Symposium on Foundations of Computer Science, (FOCS)
               2018, Paris, France, October 7-9, 2018},
  pages     = {802--813},
  year      = {2018},
  crossref  = {DBLP:conf/focs/2018},
  url       = {https://doi.org/10.1109/FOCS.2018.00081},
  doi       = {10.1109/FOCS.2018.00081},
  timestamp = {Wed, 16 Oct 2019 14:14:54 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/focs/SohlerW18},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{imagenet,
  title={Imagenet classification with deep convolutional neural networks},
  author={Krizhevsky, Alex and Sutskever, Ilya and Hinton, Geoffrey E},
  booktitle={Advances in neural information processing systems},
  pages={1097--1105},
  year={2012}
}
@inproceedings{mv10,
  author    = {Ankur Moitra and
               Gregory Valiant},
  title     = {Settling the Polynomial Learnability of Mixtures of Gaussians},
  booktitle = {51th Annual {IEEE} Symposium on Foundations of Computer Science, {FOCS}
               2010, October 23-26, 2010, Las Vegas, Nevada, {USA}},
  pages     = {93--102},
  year      = {2010},
  crossref  = {DBLP:conf/focs/2010},
  url       = {https://doi.org/10.1109/FOCS.2010.15},
  doi       = {10.1109/FOCS.2010.15},
  timestamp = {Wed, 16 Oct 2019 14:14:54 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/focs/MoitraV10},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@article{ShiMalik97,
author = {Shi, J.B. and Malik, Jitendra},
year = {1997},
month = {01},
pages = {888-905},
title = {Normalized Cuts and Image Segmentation},
volume = {22},
journal = {IEEE Trans. on Pattern Anal. and Mach. Intell.}
}

@inproceedings{NgSpectral01,
 author = {Ng, Andrew Y. and Jordan, Michael I. and Weiss, Yair},
 title = {On Spectral Clustering: Analysis and an Algorithm},
 booktitle = {Proceedings of the 14th International Conference on Neural Information Processing Systems: Natural and Synthetic},
 series = {NIPS'01},
 year = {2001},
 location = {Vancouver, British Columbia, Canada},
 pages = {849--856},
 numpages = {8},
 url = {http://dl.acm.org/citation.cfm?id=2980539.2980649},
 acmid = {2980649},
 publisher = {MIT Press},
 address = {Cambridge, MA, USA},
} 

@inproceedings{GuMi95,
     Author="Stephen Guattery and Gary L. Miller",
     Title="On the Performance of the Spectral Graph Partitioning Methods",
     Booktitle= "SODA'95",
     year="1995",
     Pages="233--242",
     Organization="ACM-SIAM",
     bib2html_rescat = {Linear Algebra,Spectral Graph Theory},   
     Thanks="CCR-9016641"}

@Article{DonathHoffman72,
  author = 	 {William Donath and Alan Hoffman},
  title = 	 {Algorithms for partitioning of graphs and computer
                  logic based on eigenvectors of connections matrices},
  journal = 	 {IBM Technical Disclosure Bulletin},
  year = 	 {1972},
  volume = 	 {15},
  OPTnumber = 	 {},
  OPTpages = 	 {},
}

@ARTICLE{Fiedler73,
    Author         = {Miroslav Fiedler},
    Journal        = {Czechoslovak Math. J.},
    Pages          = {298-305},
    Title          = {Algebraic connectivity of graphs},
    Volume         = {23},
    Number = {98},
    Year           = {1973}
}
@book{ss09,
  title={Real analysis: measure theory, integration, and Hilbert spaces},
  author={Stein, Elias M and Shakarchi, Rami},
  year={2009},
  publisher={Princeton University Press}
}
@article{kw16,
  author    = {Robert Krauthgamer and
               Tal Wagner},
  title     = {Cheeger-Type Approximation for Sparsest \emph{st}-Cut},
  journal   = {{ACM} Trans. Algorithms},
  volume    = {13},
  number    = {1},
  pages     = {14:1--14:21},
  year      = {2016},
  url       = {https://doi.org/10.1145/2996799},
  doi       = {10.1145/2996799},
  timestamp = {Tue, 06 Nov 2018 12:51:20 +0100},
  biburl    = {https://dblp.org/rec/bib/journals/talg/KrauthgamerW16},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@book{m03,
author = {Monk, Peter},
year = {2003},
month = {01},
pages = {},
title = {Finite Element Methods for Maxwell's Equations (Numerical Analysis and Scientific Computation Series)},
isbn = {0198508883}
}
@article{lw01,
  title={An Eulerian description of fluids containing visco-elastic particles},
  author={Liu, Chun and WALkINGTON, NOEL J},
  journal={Archive for rational mechanics and analysis},
  volume={159},
  number={3},
  pages={229--252},
  year={2001},
  publisher={Springer}
}
@inproceedings{dkn09,
  author    = {Ilias Diakonikolas and
               Daniel M. Kane and
               Jelani Nelson},
  title     = {Bounded Independence Fools Degree-2 Threshold Functions},
  booktitle = {51th Annual {IEEE} Symposium on Foundations of Computer Science, {FOCS}
               2010, October 23-26, 2010, Las Vegas, Nevada, {USA}},
  pages     = {11--20},
  year      = {2010},
  crossref  = {DBLP:conf/focs/2010},
  url       = {https://doi.org/10.1109/FOCS.2010.8},
  doi       = {10.1109/FOCS.2010.8},
  timestamp = {Wed, 16 Oct 2019 14:14:54 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/focs/DiakonikolasKN10},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@article{f44,
  title={The identity of weak and strong extensions of differential operators},
  author={Friedrichs, Kurt Otto},
  journal={Transactions of the American Mathematical Society},
  volume={55},
  pages={132--151},
  year={1944}
}
@article{s38,
  title={Sur un th{\'e}or{\`e}me d'analyse fonctionnelle},
  author={Soboleff, S},
  journal={Matematicheskii Sbornik},
  volume={46},
  number={3},
  pages={471--497},
  year={1938},
  publisher={Russian Academy of Sciences, Steklov Mathematical Institute of Russian~…}
}
@Book{ChungBook97,
    Author         = {F.R.K. Chung},
    Series        = {Regional Conference Series in Mathematics},
    Publisher  = {American Mathematical Society},
    Title          = {Spectral Graph Theory},
    Volume         = {92},
    Year           = {1997}
}

@incollection{Cheeger70,
  author    = {Jeff Cheeger},
  title     = {A lower bound for the smallest eigenvalue of the Laplacian},
  booktitle = {Problems in Analysis: A Symposium in Honor of Salomon Bochner},
  publisher = {Princeton Univ. Press},
  year      = {1970},
  pages     = {195--199},
  address   = {Princeton, N. J.}
}

@inproceedings{AlonM84,
 author = {Alon, N. and Milman, V. D.},
 title = {Eigenvalues, Expanders And Superconcentrators},
 booktitle = {Proceedings of the 25th Annual Symposium on Foundations of Computer Science, 1984},
 series = {FOCS '84},
 year = {1984},
 isbn = {0-8186-0591-X},
 pages = {320--322},
 numpages = {3},
 url = {http://dx.doi.org/10.1109/SFCS.1984.715931},
 doi = {10.1109/SFCS.1984.715931},
 acmid = {1398556},
 publisher = {IEEE Computer Society},
 address = {Washington, DC, USA},
}

@Article{LeeMultiway14,
  author = 	 {James R. Lee and Shayan Oveis Gharan and Luca Trevisan},
  title = 	 {Multi-way spectral partitioning and higher-order Cheeger inequalities},
  journal = 	 {Journal of the ACM},
  year = 	 {2014},
  OPTkey = 	 {},
  volume = 	 {61(6)},
  number = 	 {37},
  OPTpages = 	 {},
  OPTmonth = 	 {},
  OPTnote = 	 {},
  OPTannote = 	 {}
}
@article{l82,
  title={Least squares quantization in PCM},
  author={Lloyd, Stuart},
  journal={IEEE transactions on information theory},
  volume={28},
  number={2},
  pages={129--137},
  year={1982},
  publisher={IEEE}
}
@article{m94,
  title={Machine learning},
  author={Michie, Donald and Spiegelhalter, David J and Taylor, CC and others},
  journal={Neural and Statistical Classification},
  volume={13},
  year={1994},
  publisher={Technometrics}
}
@book{b06,
  title={Pattern recognition and machine learning},
  author={Bishop, Christopher M},
  year={2006},
  publisher={Springer Science+ Business Media}
}
@book{f01,
  title={The elements of statistical learning},
  author={Friedman, Jerome and Hastie, Trevor and Tibshirani, Robert},
  volume={1},
  number={10},
  year={2001},
  publisher={Springer series in statistics New York}
}
@inproceedings{Dyer89,
 author = {Dyer, M. and Frieze, A.},
 title = {A Random Polynomial Time Algorithm for Approximating the Volume of Convex Bodies},
 booktitle = {Proceedings of the Twenty-first Annual ACM Symposium on Theory of Computing},
 series = {STOC '89},
 year = {1989},
 isbn = {0-89791-307-8},
 location = {Seattle, Washington, USA},
 pages = {375--381},
 numpages = {7},
 url = {http://doi.acm.org/10.1145/73007.73043},
 doi = {10.1145/73007.73043},
 acmid = {73043},
 publisher = {ACM},
 address = {New York, NY, USA},
} 
@article{Buser82,
     author = {Buser, Peter},
     title = {A note on the isoperimetric constant},
     journal = {Annales scientifiques de l'\'Ecole Normale Sup\'erieure},
     publisher = {Elsevier},
     volume = {Ser. 4, 15},
     number = {2},
     year = {1982},
     pages = {213-230},
     doi = {10.24033/asens.1426},
     zbl = {0501.53030},
     mrnumber = {84e:58076},
     language = {en},
     url = {http://www.numdam.org/item/ASENS_1982_4_15_2_213_0}
}

@article{dodziuk1984difference,
  title={Difference equations, isoperimetric inequality and transience of certain random walks},
  author={Dodziuk, Jozef},
  journal={Transactions of the American Mathematical Society},
  volume={284},
  number={2},
  pages={787--794},
  year={1984}
}

@book{showalter2010hilbert,
  title={Hilbert space methods in partial differential equations},
  author={Showalter, Ralph E},
  year={2010},
  publisher={Courier Corporation}
}

@article{TrillosConsis16,
 author = {Trillos, Nicol\'{a}s Garc\'{\i}a and Slep\v{c}ev, Dejan and Von Brecht, James and Laurent, Thomas and Bresson, Xavier},
 title = {Consistency of Cheeger and Ratio Graph Cuts},
 journal = {J. Mach. Learn. Res.},
 issue_date = {January 2016},
 volume = {17},
 number = {1},
 month = {Jan},
 year = {2016},
 issn = {1532-4435},
 pages = {6268--6313},
 numpages = {46},
 url = {http://dl.acm.org/citation.cfm?id=2946645.3053463},
 acmid = {3053463},
 publisher = {JMLR.org},
 keywords = {balanced cut, consistency, data clustering, graph partitioning},
}

@article{TrillosRate15,
title={On the Rate of Convergence of Empirical Measures in $\infty$-transportation Distance},
volume={67}, DOI={10.4153/CJM-2014-044-6},
number={6}, journal={Canadian Journal of Mathematics},
publisher={Cambridge University Press},
author={Garc{\'i}a Trillos, Nicol{\'a}s
and Slep{\v{c}}ev, Dejan},
year={2015}, pages={1358–1383}
}

@Article{TrillosContin16,
author={Garc{\'i}a Trillos, Nicol{\'a}s
and Slep{\v{c}}ev, Dejan},
title="Continuum Limit of Total Variation on Point Clouds",
journal="Archive for Rational Mechanics and Analysis",
year="2016",
month= "04",
day="01",
volume="220",
number="1",
pages="193--241",
abstract={We consider point clouds obtained as random samples of a measure on a Euclidean domain. A graph representing the point cloud is obtained by assigning weights to edges based on the distance between the points they connect. Our goal is to develop mathematical tools needed to study the consistency, as the number of available data points increases, of graph-based machine learning algorithms for tasks such as clustering. In particular, we study when the cut capacity, and more generally total variation, on these graphs is a good approximation of the perimeter (total variation) in the continuum setting. We address this question in the setting of $\Gamma$-convergence. We obtain almost optimal conditions on the scaling, as the number of points increases, of the size of the neighborhood over which the points are connected by an edge for the $\Gamma$-convergence to hold. Taking of the limit is enabled by a transportation based metric which allows us to suitably compare functionals defined on different point clouds.},
issn="1432-0673",
doi="10.1007/s00205-015-0929-z",
url="https://doi.org/10.1007/s00205-015-0929-z"
}

@article{MillerHardy18,
  author    = {Gary L. Miller and
               Noel J. Walkington and
               Alex L. Wang},
  title     = {Hardy-Muckenhoupt Bounds for Laplacian Eigenvalues},
  journal   = {CoRR},
  volume    = {abs/1812.02841},
  year      = {2018},
  url       = {http://arxiv.org/abs/1812.02841},
  archivePrefix = {arXiv},
  eprint    = {1812.02841},
  timestamp = {Tue, 01 Jan 2019 15:01:25 +0100},
  biburl    = {https://dblp.org/rec/bib/journals/corr/abs-1812-02841},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{t10,
  title={The Laplacian paradigm: Emerging algorithms for massive graphs},
  author={Teng, Shang-Hua},
  booktitle={International Conference on Theory and Applications of Models of Computation},
  pages={2--14},
  year={2010},
  organization={Springer}
}

@Article{c96,
author="Chandra, Ashok K.
and Raghavan, Prabhakar
and Ruzzo, Walter L.
and Smolensky, Roman
and Tiwari, Prasoon",
title="The electrical resistance of a graph captures its commute and cover times",
journal="computational complexity",
year="1996",
month="Dec",
day="01",
volume="6",
number="4",
pages="312--340",
issn="1420-8954",
doi="10.1007/BF01270385",
url="https://doi.org/10.1007/BF01270385"
}

@article{f10,
  title={Community detection in graphs},
  author={Fortunato, Santo},
  journal={Physics reports},
  volume={486},
  number={3-5},
  pages={75--174},
  year={2010},
  publisher={Elsevier}
}
@inproceedings{e96,
	Acmid = {3001507},
	Author = {Ester, Martin and Kriegel, Hans-Peter and Sander, Jorg and Xu, Xiaowei},
	Booktitle = {Proceedings of the Second International Conference on Knowledge Discovery and Data Mining},
	Keywords = {arbitrary shape of clusters, clustering algorithms, efficiency on large spatial databases, handling nlj4-275oise},
	Location = {Portland, Oregon},
	Numpages = {6},
	Pages = {226--231},
	Publisher = {AAAI Press},
	Series = {KDD'96},
	Title = {A Density-based Algorithm for Discovering Clusters a
	     Density-based Algorithm for Discovering Clusters in Large Spatial Databases with Noise},
	Url = {http://dl.acm.org/citation.cfm?id=3001460.3001507},
	Year = {1996},
	Bdsk-Url-1 = {http://dl.acm.org/citation.cfm?id=3001460.3001507}}


@inproceedings{bjw19,
  author    = {Ainesh Bakshi and
               Rajesh Jayaram and
               David P. Woodruff},
  title     = {Learning Two Layer Rectified Neural Networks in Polynomial Time},
  booktitle = {Conference on Learning Theory, {COLT} 2019, 25-28 June 2019, Phoenix,
               AZ, {USA}},
  pages     = {195--268},
  year      = {2019},
  crossref  = {DBLP:conf/colt/2019},
  url       = {http://proceedings.mlr.press/v99/bakshi19a.html},
  timestamp = {Mon, 08 Jul 2019 16:13:41 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/colt/BakshiJW19},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@article{von2007tutorial,
  title={A tutorial on spectral clustering},
  author={Von Luxburg, Ulrike},
  journal={Statistics and computing},
  volume={17},
  number={4},
  pages={395--416},
  year={2007},
  publisher={Springer}
}


@incollection{awasthi2012improved,
  title={Improved spectral-norm bounds for clustering},
  author={Awasthi, Pranjal and Sheffet, Or},
  booktitle={Approximation, Randomization, and Combinatorial Optimization. Algorithms and Techniques},
  pages={37--49},
  year={2012},
  publisher={Springer}
}

@inproceedings{moitra2010settling,
  title={Settling the polynomial learnability of mixtures of gaussians},
  author={Moitra, Ankur and Valiant, Gregory},
  booktitle={2010 IEEE 51st Annual Symposium on Foundations of Computer Science},
  pages={93--102},
  year={2010},
  organization={IEEE}
}

@book{jolliffe2011principal,
  title={Principal component analysis},
  author={Jolliffe, Ian},
  year={2011},
  publisher={Springer}
}

@article{muckenhoupt1972hardy,
  title={Hardy's inequality with weights},
  author={Muckenhoupt, Benjamin},
  journal={Studia Mathematica},
  volume={44},
  number={1},
  pages={31--38},
  year={1972}
}

@article{colbois2018eigenvalues,
  title={Eigenvalues of elliptic operators with density},
  author={Colbois, Bruno and Provenzano, Luigi},
  journal={Calculus of Variations and Partial Differential Equations},
  volume={57},
  number={2},
  pages={36},
  year={2018},
  publisher={Springer}
}

@article{colbois2019spectrum,
  title={Spectrum of the Laplacian with weights},
  author={Colbois, Bruno and El Soufi, Ahmad},
  journal={Annals of Global Analysis and Geometry},
  volume={55},
  number={2},
  pages={149--180},
  year={2019},
  publisher={Springer}
}

@inproceedings{Ge2018,
 author = {Ge, Rong and Lee, Holden and Risteski, Andrej},
 title = {Beyond Log-concavity: Provable Guarantees for Sampling Multi-modal Distributions Using Simulated Tempering Langevin Monte Carlo},
 booktitle = {Proceedings of the 32Nd International Conference on Neural Information Processing Systems},
 series = {NIPS'18},
 year = {2018},
 location = {Montr\&\#233;al, Canada},
 pages = {7858--7867},
 numpages = {10},
 url = {http://dl.acm.org/citation.cfm?id=3327757.3327882},
 acmid = {3327882},
 publisher = {Curran Associates Inc.},
 address = {USA},
}
@inproceedings{ACL06,
  title={Local graph partitioning using pagerank vectors},
  author={Andersen, Reid and Chung, Fan and Lang, Kevin},
  booktitle={2006 47th Annual IEEE Symposium on Foundations of Computer Science (FOCS'06)},
  pages={475--486},
  year={2006},
  organization={IEEE}
}
@inproceedings{Schild18,
  title={A Schur Complement Cheeger Inequality},
  author={Schild, Aaron},
  series={ITCS '19},
  year={2018}
}
@book{hk00,
  title={Sobolev met poincar{\'e}},
  author={Haj{\l}asz, Piotr and Koskela, Pekka},
  volume={688},
  year={2000},
  publisher={American Mathematical Soc.}
}

@book{vsc08,
  title={Analysis and geometry on groups},
  author={Varopoulos, Nicholas T and Saloff-Coste, Laurent and Coulhon, Thierry},
  volume={100},
  year={2008},
  publisher={Cambridge university press}
}
@article{Lee2014,
  title={Multiway spectral partitioning and higher-order cheeger inequalities},
  author={Lee, James R and Gharan, Shayan Oveis and Trevisan, Luca},
  journal={Journal of the ACM (JACM)},
  volume={61},
  number={6},
  pages={37},
  year={2014},
  publisher={ACM}
}
@inproceedings{Louis12,
  title={Many sparse cuts via higher eigenvalues},
  author={Louis, Anand and Raghavendra, Prasad and Tetali, Prasad and Vempala, Santosh},
  booktitle={Proceedings of the forty-fourth annual ACM symposium on Theory of computing},
   series = {FOCS 2012},
  pages={1131--1140},
  year={2012},
  organization={ACM}
}
@inproceedings{Trevisan09,
  title={Max cut and the smallest eigenvalue},
  author={Trevisan, Luca},
  series={STOC '09},
  publisher={ACM}
}

@article{Bobkov97,
  title={Isoperimetric constants for product probability measures},
  author={Bobkov, Sergey G and Houdr{\'e}, Christian},
  journal={The Annals of Probability},
  pages={184--205},
  year={1997},
  publisher={JSTOR}
}

@inproceedings{Andersen09,
  title={Finding sparse cuts locally using evolving sets},
  author={Andersen, Reid and Peres, Yuval},
  booktitle={Proceedings of the forty-first annual ACM symposium on Theory of computing},
  series={STOC '09},
  pages={235--244},
  year={2009},
  organization={ACM}
}

@INPROCEEDINGS{LV17,
author={Y. T. {Lee} and S. S. {Vempala}}, 
booktitle={2017 IEEE 58th Annual Symposium on Foundations of Computer Science (FOCS)}, 
 series = {FOCS 2017},
title={Eldan's Stochastic Localization and the KLS Hyperplane Conjecture: An Improved Lower Bound for Expansion}, 
year={2017}, 
volume={}, 
number={}, 
pages={998-1007}, 
doi={10.1109/FOCS.2017.96}, 
ISSN={}, 
month={Oct},
}

@article{Dyer91,
 author = {Dyer, Martin and Frieze, Alan and Kannan, Ravi},
 title = {A Random Polynomial-time Algorithm for Approximating the Volume of Convex Bodies},
 journal = {J. ACM},
 issue_date = {Jan. 1991},
 volume = {38},
 number = {1},
 month = jan,
 year = {1991},
 issn = {0004-5411},
 pages = {1--17},
 numpages = {17},
 url = {http://doi.acm.org/10.1145/102782.102783},
 doi = {10.1145/102782.102783},
 acmid = {102783},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {convex sets, random walks, sampling, volume},
}
@article{Gromov83,
  title={A topological application of the isoperimetric inequality},
  author={Gromov, Mikhail and Milman, Vitali D},
  journal={American Journal of Mathematics},
  volume={105},
  number={4},
  pages={843--854},
  year={1983},
  publisher={JSTOR}
}
@article{Milman09,
  title={On the role of convexity in isoperimetry, spectral gap and concentration},
  author={Milman, Emanuel},
  journal={Inventiones mathematicae},
  volume={177},
  number={1},
  pages={1--43},
  year={2009},
  publisher={Springer}
} 

@article{KLS95,
  author    = {Ravi Kannan and
               L{\'{a}}szl{\'{o}} Lov{\'{a}}sz and
               Mikl{\'{o}}s Simonovits},
  title     = {Isoperimetric Problems for Convex Bodies and a Localization Lemama},
  journal   = {Discrete {\&} Computational Geometry},
  volume    = {13},
  pages     = {541--559},
  year      = {1995},
  url       = {https://doi.org/10.1007/BF02574061},
  doi       = {10.1007/BF02574061},
  timestamp = {Tue, 06 Aug 2019 16:18:34 +0200},
  biburl    = {https://dblp.org/rec/bib/journals/dcg/KannanLS95},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{Lovasz90,
 author = {Lovasz, L. and Simonovits, M.},
 title = {The Mixing Rate of Markov Chains, an Isoperimetric Inequality, and Computing the Volume},
 booktitle = {Proceedings of the 31st Annual Symposium on
   Foundations of Computer Science (FOCS)},
 series = {FOCS '90},
 year = {1990},
 isbn = {0-8186-2082-X},
 pages = {346--354 vol. 1},
 url = {https://doi.org/10.1109/FSCS.1990.89553},
 doi = {10.1109/FSCS.1990.89553},
 acmid = {1398775},
 publisher = {IEEE Computer Society},
 address = {Washington, DC, USA},
 keywords = {Markov chains, conductance, convex body, isoperimetric inequality, mixing rate, running-time, time-reversible},
} 
@inproceedings{Lee18,
 author = {Lee, Yin Tat and Vempala, Santosh S.},
 title = {Stochastic Localization + Stieltjes Barrier = Tight Bound for log-Sobolev},
 booktitle = {Proceedings of the 50th Annual ACM SIGACT Symposium on Theory of Computing},
 series = {STOC 2018},
 year = {2018},
 isbn = {978-1-4503-5559-9},
 location = {Los Angeles, CA, USA},
 pages = {1122--1129},
 numpages = {8},
 url = {http://doi.acm.org/10.1145/3188745.3188866},
 doi = {10.1145/3188745.3188866},
 acmid = {3188866},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {Log-Sobolev constant, Logconcave densities, Stieltjes barrier, ball walk, stochastic localization},
} 

@misc{Lee18Survey,
    title={The Kannan-Lovász-Simonovits Conjecture},
    author={Yin Tat Lee and Santosh S. Vempala},
    year={2018},
    eprint={1807.03465},
    archivePrefix={arXiv},
    primaryClass={math.PR}
} 

@inproceedings{Kwok2016,
 author = {Kwok, Tsz Chiu and Lau, Lap Chi and Lee, Yin Tat},
 title = {Improved Cheeger's Inequality and Analysis of Local Graph Partitioning Using Vertex Expansion and Expansion Profile},
 booktitle = {Proceedings of the Twenty-seventh Annual ACM-SIAM Symposium on Discrete Algorithms},
 series = {SODA '16},
 year = {2016},
 isbn = {978-1-611974-33-1},
 location = {Arlington, Virginia},
 pages = {1848--1861},
 numpages = {14},
 url = {http://dl.acm.org/citation.cfm?id=2884435.2884564},
 acmid = {2884564},
 publisher = {Society for Industrial and Applied Mathematics},
 address = {Philadelphia, PA, USA},
} 

@article{belkin2004semisup,
 author = {Belkin, Mikhail and Niyogi, Partha},
 title = {Semi-Supervised Learning on Riemannian Manifolds},
 journal = {Mach. Learn.},
 volume = {56},
 number = {1-3},
 month = jun,
 year = {2004},
 issn = {0885-6125},
 pages = {209--239},
 numpages = {31},
 url = {https://doi.org/10.1023/B:MACH.0000033120.25363.1e},
 doi = {10.1023/B:MACH.0000033120.25363.1e},
 acmid = {1007769},
 publisher = {Kluwer Academic Publishers},
 address = {Norwell, MA, USA},
 keywords = {graph laplacian, graph regularization, laplace operator, manifold learning, semi-supervised learning},
} 

@article{von2008consistency,
  title={Consistency of spectral clustering},
  author={Von Luxburg, Ulrike and Belkin, Mikhail and Bousquet, Olivier},
  journal={The Annals of Statistics},
  pages={555--586},
  year={2008},
  publisher={JSTOR}
}

@article{rosasco2010learning,
  title={On learning with integral operators},
  author={Rosasco, Lorenzo and Belkin, Mikhail and Vito, Ernesto De},
  journal={Journal of Machine Learning Research},
  volume={11},
  number={Feb},
  pages={905--934},
  year={2010}
}

@inproceedings{belkin2005towards,
  title={Towards a theoretical foundation for Laplacian-based manifold methods},
  author={Belkin, Mikhail and Niyogi, Partha},
  booktitle={International Conference on Computational Learning Theory},
  pages={486--500},
  year={2005},
  organization={Springer}
}

@inproceedings{hein2005graphs,
  title={From graphs to manifolds--weak and strong pointwise consistency of graph Laplacians},
  author={Hein, Matthias and Audibert, Jean-Yves and Von Luxburg, Ulrike},
  booktitle={International Conference on Computational Learning Theory},
  pages={470--485},
  year={2005},
  organization={Springer}
}

@inproceedings{belkin2007convergence,
  title={Convergence of Laplacian eigenmaps},
  author={Belkin, Mikhail and Niyogi, Partha},
  booktitle={Advances in Neural Information Processing Systems},
  pages={129--136},
  year={2007}
}

@inproceedings{hein2006uniform,
  title={Uniform convergence of adaptive graph-based regularization},
  author={Hein, Matthias},
  booktitle={International Conference on Computational Learning Theory},
  pages={50--64},
  year={2006},
  organization={Springer}
}

@Book{EvansNumer99,
  author = 	 {Gwynne Evans and Jonathan M. Blackledge and P. Yardley},
  ALTeditor = 	 {},
  title = 	 {Numerical Methods for Partial Differential Equations},
  publisher = 	 {Springer},
  year = 	 {1999},
  OPTkey = 	 {},
  OPTannote = 	 {}
}

@Book{EvansMeasure15,
  author = 	 {Lawrence C. Evans and Ronald F. Gariepy},
  ALTeditor = 	 {},
  title = 	 {Measure Theory and Fine Properties of Functions},
  publisher = 	 {CRC Press},
  year = 	 {2015},
  OPTkey = 	 {},
  OPTannote = 	 {}
}

@misc{TrillosVariational15,
  Author = {Nicolás García Trillos and Dejan Slepčev},
  Title = {A variational approach to the consistency of spectral clustering},
  Year = {2015},
  Eprint = {arXiv:1508.01928},
}

@article{parini2011introduction,
  title={An introduction to the Cheeger problem},
  author={Parini, Enea},
  journal={Surv. Math. Appl.},
  volume={6},
  pages={9--21},
  year={2011}
}

@article{betta2008weighted,
  title={Weighted isoperimetric inequalities on $\mathbb{R}^n$ and applications to rearrangements},
  author={Betta, M Francesca and Brock, Friedemann and Mercaldo, Anna and Posteraro, M Rosaria},
  journal={Mathematische Nachrichten},
  volume={281},
  number={4},
  pages={466--498},
  year={2008},
  publisher={Wiley Online Library}
}


==> buser/buser-definitions.tex <==
In this section we are given three positive constants
$\alpha,\beta,\gamma$ and an $L$-Lipschitz density function 
$\rho:\RR^d \to \RR_+$ that in $\alpha$-integrable over all of $\RR^d$.
Further we have a partition $A,B$ of $\RR^d$ into two measurable sets.

\begin{definition}
For a measurable set $A\subseteq \bbR^d$, define
\begin{align*}
\abs{A}_\alpha \coloneqq \int_A \rho^\alpha(x)\,dx.
\end{align*}
\end{definition}

We define the weight of the boundary distributionally~\cite{betta2008weighted,parini2011introduction}.
\begin{definition}
\label{def:betaBdy}
For $A$ a set who's $\rho^{\beta}$ weighted perimeter is finite, define
\begin{align*}
\abs{\boundary A}_\beta \coloneqq \sup\set{\int_\bbR^d \chi_A(x)
  \div(\rho^\beta (x) \phi(x))\,dx\smid \phi\in C_c^1(\bbR^d),\, \norm{\phi}_{\infty}\leq 1}.
\end{align*}
\end{definition}

\begin{remark}
We note that this definition of the boundary weight corresponds to the
intuitive definition when $\boundary A$ is sufficiently
regular. Specifically, if $A$ has smooth boundary and
has finite perimeter in $K$ for every compact $K\subseteq U$, then,
\begin{align*}
\abs{\boundary A}_\beta = \int_{\boundary A} \rho^\beta(x)\,d \mc H^{n-1}.
\end{align*}
\end{remark}


\begin{definition}
  Let $A$ be a sat with $\rho^{\beta}$ weighted finite perimeter such
  that $\abs{A}_\alpha,\abs{\bbR^d\setminus A}_\alpha >0$. The
  \textit{isoperimetric ratio} of the cut induced by $A,B$ is
\begin{align*}
\Phi(A) &\coloneqq \frac{\abs{\boundary A}_\beta}{\min\left(\abs{A}_\alpha,\abs{B}_\alpha\right)}
\end{align*}

and the \textit{isoperimetric constant} of $\rho$ is
\begin{align*}
\Phi(\rho)\coloneqq \inf_{A \subset \RR^d} \Phi(A).
\end{align*}
Here, $A$ is taken over sets of $\rho$-finite perimeter such that $\abs{A}_\alpha,\abs{B}_\alpha>0$.
\end{definition}

Again we define $\lambda_2$ variationally.
\begin{definition}
Let $u\in W^{1,2}$. The \textit{Rayleigh quotient} of $u$ is
\begin{align*}
R(u) &= \frac{\int \rho^\gamma\norm{\grad u}^2\,dx}{\int \rho^\alpha u^2\,dx}
\end{align*}
and the \textit{second eigenvalue of the Laplacian} on $\RR^d$ with weight $\rho$ is
\begin{align*}
\lambda_2(\rho) &\coloneqq \inf_{u\in W^{1,2}}\set{R(u) \smid \int \rho^\alpha u \,dx = 0,\, u\neq 0}.
\end{align*}
\end{definition}




==> changing-beta/changing-beta.tex <==
\section{The Effects of Changing $\beta$ on $(1,\beta)$-sparse cuts}
\label{sec:changing-beta}


==> experiments.tex <==
%!TEX root = ms.tex

\section{Experimental results}
\label{sec:experiments}
In this section we describe an algorithm inspired by Theorem~\ref{thm:main} and show some numerical results. In particular, we observe how the algorithm performs for different choices of $(\alpha,\beta,\gamma)$.

Let $\Omega=(0,l)\times(0,w)\subseteq\RR^2$. We assume we are
explicitly given a weight $\rho:\Omega\to\RR_{\geq 0}$ and a small grid size $0<h\ll \min(l,w)$. We will use a finite element method to approximately find an eigenfunction of the Laplacian. Then, we will search for a small cut among the level sets of the eigenfunction.

Let $n = \ceil{l/h}$ and $m=\ceil{w/h}$. Let the vertices be $V=\set{0,1,\dots,n}\times\set{0,1,\dots,m}$. We will think of vertex $(i,j)$ as representing the $h\times h$ square $\Omega_{i,j}=((i- 1/2) h, (i+1/2) h) \times ((j- 1/2) h, (j+1/2) h)\subseteq \Omega$. On the boundary, the set $\Omega_{i,j}$ may be only part of an $h\times h$ square. Define
\begin{align*}
\mu_{i,j}= \abs{\Omega_{i,j}}\rho^\alpha(ih, jh)\approx \int_{\Omega_{i,j}}\rho^\alpha(x,y)\,dx\,dy.
\end{align*}

We will connect each vertex $(i,j)$ to its four neighbors. Suppose $\Omega_{i,j}$ touches $\Omega_{i',j'}$ along the edge $E$. Then define
\begin{align*}
\kappa((i,j),(i',j')) = \frac{\abs{E}}{h} \rho^\gamma\left(\frac{i+i'}{2}, \frac{j+j'}{2}\right)\approx \frac{1}{h}\int_E \rho^\gamma(x,y)\,dx\,dy.
\end{align*}
we will approximate the second eigenvalue of the continuous Laplacian by computing the second eigenvalue of the graph with edge weights $\kappa$ and vertex weights $\mu$.

Associate to each edge the cut cost
\begin{align*}
\tau((i,j),(i',j')) = \abs{E} \rho^\beta\left(\frac{i+i'}{2}, \frac{j+j'}{2}\right)\approx \int_E \rho^\beta(x,y)\,dx\,dy.
\end{align*}
Let $A\subseteq V$.
We will approximate the sparsity of the cut $(\Omega_A,\Omega_A^c)$ where $\Omega_A = \bigcup_{(i,j)\in A} \Omega_{i,j}\subseteq \Omega$ by
\begin{align*}
\Phi(\Omega_A,\Omega_A^c) \approx \Phi(A, A^c) = \frac{\sum_{e\in E(A, A^c)} \tau_e}{\min(\mu(A),\mu(A^c))}
\end{align*}
where $E(A,A^c)$ is the set of edges with exactly one end point in $A$ and $\mu(A) = \sum_{v\in A} \mu_v$.

Consider the following algorithm.
\begin{algorithm}
\label{alg:single_cut}
	Given $\rho:\Omega\to\RR_{\geq 0}$,  $h>0$, and $\alpha,\beta,\gamma>0$
	\begin{enumerate}
	 	\item Let $L$ be the Laplacian matrix with edge weights $\kappa$ and let $M=\diag(\mu)$
	 	\item (Approximately) find a vector $x$ corresponding to the second eigenvalue of $Lx = \lambda Mx$
	 	\item Let $A_t = \set{v\in V \smid x_v >t}$ for $t\in\RR$ and let $A$ be the minimizer of $\Phi$ among sets of this form 
	 	\item Output $\Omega_A$
	 \end{enumerate} 
\end{algorithm}

Experimentally, we find that the algorithm above often cuts off small corners. This is particular problematic when $\rho$ takes on small values near the corners of $\Omega$. We instead test an iterative version of the above algorithm.

\begin{algorithm}
\label{alg:multiple_cuts}
	Given $\rho:\Omega\to\RR_{\geq 0}$, $h>0$, and $\alpha,\beta,\gamma>0$
	\begin{enumerate}
		\item Let $\Omega_0 = \Omega$, $k=0$
		\item While $\mu(\Omega_k)\geq \frac{9}{10} \mu(\Omega)$
		\begin{enumerate}
			\item Partition $\Omega_k$ using Algorithm \ref{alg:single_cut}
			\item Let $A$ be the connected component with the most weight
			\item Set $k = k+1$ and let $\Omega_k = \Omega_A$
		\end{enumerate}
		\item Return $\Omega_k$
	\end{enumerate}
\end{algorithm}

In Figure \ref{fig:alg}, we show the output of Algorithm \ref{alg:multiple_cuts} for the choices $(\alpha,\beta,\gamma)=(1,1,1)$ and $(1,2,3)$ on different toy examples: noisy half moons, noisy concentric circles, and a long valley. We note that the output of the algorithm varies drastically for the different choices of $(\alpha,\beta,\gamma)$.

\begin{figure}
\centering
\subfloat[Noisy half moons]{
  \includegraphics[width=4.5in]{images/moons.png}
}\hspace{0mm}
\subfloat[Noisy concentric circles]{
  \includegraphics[width=4.5in]{images/circles.png}
}\hspace{0mm}
\subfloat[Long valley]{
  \includegraphics[width=4.5in]{images/trough.png}
}
\caption{
In each row, the first image shows the heat map of a fixed $\rho:\Omega\to\RR_>0$, the second and third images shows the set $\Omega_k$ returned by Algorithm \ref{alg:multiple_cuts} (displayed in black) for the choices $(\alpha,\beta,\gamma)$ of $(1,1,1)$ and $(1,2,3)$ respectively.
 }
\label{fig:alg}
\end{figure}




==> introduction/motivation.tex <==
\subsection{Motivation}

Our new method of generating clustering problems is inspired by two
separate lines of work, which both pioneer the use of variational
methods for
classical machine learning problems: the first is the work of von
Luxburg, Belkin, and Bosquet~\cite{von2008consistency} on determining how 
spectral clusering algorithms of Ng, Jordan, and
Weiss~\cite{NgSpectral01} (over 10,000 citations) behave as the number
of samples grows large. This was refined by Trillos and
Slepcev~\cite{TrillosRate15, TrillosVariational15}.
The second line of work models optimization algorithms like gradient descent
as continuous-time differential equations. The latter method was introduced
by Su, Boyd, and Candes in~\cite{SuNesterov14} and expanded upon by
Wibisono, Wilson, and Jordan in ~\cite{WibisonoGradient16}.


The first line of work on spectral clustering advances the idea that
clustering should be seen as a discrete analog of a partitioning process
on an underlying probability density. The work of Trillos and
Slepcev~\cite{TrillosVariational15} proves that the
spectral clustering methods of Ng, Jordan, and Weiss converge to what we
will call a $(1,2)$ spectral sweep cut of a probability density
function, as the number of samples grows large. We will define these
sweep cuts formally in Section~\ref{sec:density-contribution}. We note
that Trillos and Slepcev
make certain regularity assumptions on the probability density (such as
being bounded above and below) in order to guarantee their results. For
readers interested in seeing the extent of these assumptions, we refer
them to their paper at~\cite{TrillosVariational15}.

Our work differs from the work of Trillos and Slepcev, and the spectral
clustering algorithm of Ng et al, in a significant way: first, while
Trillos and Slepcev proved that the
spectral clustering algorithm of Ng. et al converge to a $(1,2)$ spectral
sweep cut of the underlying probability density as the number of samples
grow large, there are currently no guarantees on the sparsity of such
cuts.
In our work, we propose instead to cluster
using a $(1,3)$ spectral sweep cut on the probability density. We will show that such a sweep cut has
desirable sparse-cut or isoperimetry properties on any $L$-Lipschitz
probability density, for appropriately
defined notions of cut sparsity. We will also show that $(1,2)$ spectral
sweep cuts cannot have nice sparse-cut guarantees.

Meanwhile, the work of Su, Boyd, and Candes~\cite{SuNesterov14} involves taking a
discrete optimization algorithm, such as accelerated gradient descent, and
finding a continuous time algorithm that this descent method converges
to given extremely small step sizes.  This approach was expanded
upon by Wibisono, Wilson, and Jordan~\cite{WibisonoGradient16}, where they generated new
gradient descent methods by first looking at continuous descent
processes with desirable properties,
and then writing down discretizations. This strategy of first looking at
continuous algorithms and then discretizing them, inspires our new
strategy for generating clustering algorithms.

These two past works motivate our clustering strategy: first, we find
desirable partitionings for continuous probability density functions, and then we
write down discretizations. In the rest of this introduction, we
formally define our notions of sparsity and spectral sweep cuts,
write down our core theorems, discuss past work, and carefully enumerate
our proof and theoretical contributions.



==> introduction/old-definitions.tex <==
\subsection{Definitions}\label{sec:definitions}
Using the upcoming definitions, we make
Theorem~\ref{thm:informal} precise. These definitions are
inspired by the definition of fundamental eigenvalues and
isoperimetric cuts for graphs and manifolds.

\subsubsection{Isoperimetric Cuts of Distributions}
Let $\alpha$ and $\beta$ be two arbitrary non-negative constants.
Let $\rho: \Re^d \rightarrow \Re_{\geq 0}$.

Let $A \subset \bbR^d$. 
Let $u\coloneqq \chi_A$, the characteristic function of $A$, i.e., $u(x) =
1$ if $x \in A$ and zero otherwise.  We say that $A$ has
\textbf{finite $\beta$-perimeter} if there exists a sequence of
functions $\{u_n\}_{n=1}^\infty \subset C^\infty(\Re^d)$ with $u_n
\rightarrow u$ in $\Lone$ for which \cite{EvansMeasure15}
\[
\abs{\boundary A}_\beta
= \lim_{n \rightarrow \infty} \int  \rho^\beta|\nabla u_n|
\eqqcolon  \int  \rho^\beta|\nabla u|
\]
exists and is finite.

Assuming $\int_{A} \rho^\alpha u \leq \int_{\bbR^d - A}
\rho^\alpha u $ (and interchanging $A$ and $B$ if otherwise), we define the
\textbf{$(\alpha, \beta)$-sparsity} of the cut defined by $A$
to be $\Phi_{\alpha, \beta}(A)$ where:
\[
  \Phi_{\alpha, \beta} (A) 
:= \frac{\int \rho^\beta |\nabla u|}{\int \rho^\alpha u}
= \lim_{n\to\infty}\frac{\int \rho^\beta\abs{\grad u_n}}{\int \rho^\alpha \abs{u_n}}.
\]
The \textbf{$(\alpha, \beta)$-isoperimetric cut} of the
distribution $\rho$ is the set $A \subset \Re^d$ that minimizes $\Phi_{\alpha,
\beta}(A)$. When $\alpha, \beta$ are clear from context, we
simply call it the isoperimetric cut and denote it as $\Phi$.
\subsubsection{Eigenvalues and $(\alpha, \gamma)$-Rayleigh Quotients of Distributions}
Define the \textbf{$(\alpha, \gamma)$-Rayleigh quotient} of $u$ with
respect to $\rho:\Re^d \to \Re_{\geq 0}$ as:

\[
  R_{\alpha, \gamma}(u) \coloneqq \frac{\int_{\Re^d} \rho^\gamma
  |\nabla u|^2}{\int_{\Re^d} \rho^{\alpha}|u|^2} 
\]

Define a \textbf{$(\alpha, \gamma)$-principal eigenvalue} of $\rho$ to be
$\lambda_2$, where:

\[ \lambda_2 := \inf_{\int \rho^\alpha u = 0} R_{\alpha, \gamma}(u). \]

When $(\alpha, \gamma)$ is clear, we simply refer to the above
terms as Rayleigh quotient and eigenvalue respectively. In this
case, we denote $R_{\alpha, \gamma}(u) = R(u)$.

Finally, define a \textbf{$(\alpha, \gamma)$-principal eigenfunction} of
$\rho$ to be a function $u$ such that $R_{\alpha, \gamma}(u) =
\lambda_2$.

We note that the eigenvalue $\lambda_2$ can also be defined in
terms of a partial differential equation: 
\begin{align*}
-\div\left(\rho^\gamma \grad f\right) = \lambda \rho^\alpha f,
\end{align*}
However, for our
purposes, the Rayleigh quotient definition suffices.

Throughout our paper, we will use the variables $\alpha, \beta,
\gamma$. It may be helpful for the reader to set these numbers to be $1, 2,$ and $3$
repsectively, as this is the simplest setting of these variables
in which we can recover our main theorems.

\subsubsection{Additional Definitions}
A function $\rho: \Re^d \to \Re_{\geq 0}$ is
\textbf{$L$-Lipschitz} if $|\rho(x)-\rho(y)|_2 \leq L|x-y|_2$ for
all $x, y \in \Re^d.$

A function is $\rho:\Re^d \to \Re_{\geq 0}$ is
\textbf{$\alpha$-integrable} if $\int_{\Re^d} \rho^\alpha$ is
well defined and finite. Throughout this paper, we assume $\rho$
is always $\alpha$-integrable.


==> introduction/theorem.tex <==
\subsection{Main Theorems}
We are now ready to state a formal version of
Theorem~\ref{thm:informal}.
\begin{theorem}\label{thm:formal} (Distributional Cheeger)
For an $L$-Lipschitz function $\rho: \Re^d
  \rightarrow \Re_{\geq 0}$, for variables $(\alpha, \beta, \gamma)$
  where $\beta = \alpha +1$ and $\gamma = \alpha+2$, we have:

\[ \Phi^2/4 \leq \lambda_2 \leq 3 \cdot 2^{\beta+1}d \cdot
\max(L\Phi ,2^{\beta + 1}\Phi^2). \]
  where $\lambda_2$ is the $(\alpha, \gamma)$ eigenvalue of $\rho$,
  and $\Phi$ is the $(\alpha, \beta)$-sparsity of the $(\alpha,
  \beta)$-isoperimetric
  cut for $\rho$.
\end{theorem}
When $(\alpha = 1, \beta = 2, \gamma = 3)$, we have:
\[ \Phi^2/4 \leq \lambda_2 \leq 24d 
\max(L\Phi, 8\Phi^2). \]

We denote the lower bound on $\lambda_2$ as the \textbf{Cheeger
Inequality}, as this is the bound that Cheeger
proved for manifolds~\cite{Cheeger70}. We call the upper bound on
$\lambda_2$ the \textbf{Buser inequality}
~\cite{Buser82}.
Assuming constant dimension, both the Buser inequality and the
Cheeger inequality in Theorem~\ref{thm:formal}
are tight up to constant factors. We will see this in
Section~\ref{sec:examples}.

Note that theorem~\ref{thm:formal} has a partial converse: when $\alpha, \beta,
\gamma$ are set improperly, no such Cheeger-like statement can
hold.
\begin{lemma}\label{lem:converse}
If $\gamma - 2 \leq \alpha$, then
  there exists $\rho: \Re^d \to \Re_{\geq 0}$ which is a $1$-Lipschitz function in
  $1$ dimension, such that either:
  \[
    \lambda_2 =  o(\Phi^2)
    \]
  or 
  \[ 
    \max(\Phi, \Phi^2) = o(\lambda_2).
  \]
\end{lemma}
Together, Theorem~\ref{thm:formal} and Lemma~\ref{lem:converse}
give restrictions on what $(\alpha, \beta, \gamma)$ must
equal, for both a Cheeger and Buser inequality to hold on an $L$-Lipschitz
distribution.


==> introduction/tim-introduction.tex <==
\section{Introduction}

Clustering, the task of
partitioning data into groups, is one of the fundamental tasks
in machine learning~\cite{bishopBook, NgSpectral01, e96, kk10clustering, sw18}.
The data that practitioners seek to cluster is commonly modeled as samples from a probability density function,
an assumption foundational in theory, statistics, and AI~\cite{bishopBook,
TrillosContin16, bc17focs, mv10, Ge2018}. 
A clustering algorithm on data drawn from a probability density function
should ideally converge to a partitioning of the
probability density function, as the number of samples grows
large~\cite{von2008consistency, TrillosVariational15,
TrillosContin16}.
 
% As the sample count grows, simple tasks like 2-way clustering will
% ideally converge to a cut of the underlying probability density.
% Surprisingly, there are almost no clustering algorithms in the machine
% learning literature that give any guarantees on the cut quality of the
% probability density, absent strong parametric assumptions on the
% density function~\footnote{Strong parametric assumptions may include:
% being a mixture of Gaussians, or a mixture of log-concave
% distributions.}. 

In this paper, we outline a new strategy for
clustering. We then make progress on implementing this strategy. We
build clustering algorithms by addressing the following two questions:

\begin{enumerate}
  \item How can we partition probability density functions? How can we
    do this so
    that two data points drawn from the same part of the partition are
    likely to be similar, and two data points drawn from different parts of the partition
    are likely to be dissimilar?

  \item What clustering algorithms converge to such a partition, 
    as the number of samples from the density function grows large?
\end{enumerate}

In this paper, we address both points, with emphasis on the first.  We
focus on the special case of $2$-way partitioning, which can be seen as
finding a good cut on the probability density function. First, we
propose a new notion of sparse (or isoperimetric)
cuts on density functions. We call this an $(\alpha, \beta)$-sparse cut,
for real parameters $\alpha$ and $\beta$. Next, we propose a new notion of spectral
sweep cuts on probability densities, called a $(\alpha,
\gamma)$-spectral sweep cut, for real parameters $\alpha$ and $\gamma$.
We show that a $(\alpha, \gamma)$-spectral sweep cut provably
approximates an $(\alpha, \beta)$-sparse cut when
$\beta = \alpha+1$ and $\gamma=\alpha+2$. In particular, $\alpha = 1, \beta = 2,
\gamma=3$ is such a setting.
Our result holds for any $L$-Lipschitz
probability density function on $\mathbb{R}^d$, for any $d$. 
We will give evidence that partitioning probability densities via
$(\alpha=1, \beta=2)$-sparse cuts agrees with the machine learning
intuition that data drawn from the same part of the partition are
similar, and data drawn from different parts of the partition are
dissimilar.  
% To our
% knowledge, this is the first result we know of that gives
% theoretical guarantees on a partitioning method for probability density
% functions, where these density functions do not have any strong
% parametric assumptions\footnote{Examples of parametric assumptions
% include: assuming that a density function
% is the mixture of finitely many log-concave functions, or a mixture of
% Gaussians.}.

The key mathematical contribution of this paper is a new Cheeger and Buser
inequality for probability density functions, which we use to prove
that $(\alpha,\gamma)$-spectral sweep cuts approximate $(\alpha,
\beta)$-sparse cuts on probability
density functions for the aforementioned settings of $\alpha, \beta, \gamma$.
These inequalities
are inspired by the Cheeger and Buser inequalities on graphs and
manifolds~\cite{AlonM84, Cheeger70, Buser82}, which have received
considerable attention in graph algorithms and machine
learning~\cite{ChungBook97, SpielmanTeng2004, Orecchia08, Orecchia2011,
kw16, belkin2004semisup}. These new inequalities do not directly follow
from either the graph or manifold Cheeger inequalities,
something we detail in Section~\ref{sec:cheeger-buser-difficulties}.
We note that our Cheeger and Buser inequalities for probability density
functions require a careful definition of eigenvalue and
sparse/isoperimetric cut for density functions: existing definitions
lead to false inequalities. 
% The Cheeger and Buser inequality for
% probability density functions is the first new Cheeger and Buser
% inequality since Alon and Milman's development of graph Cheeger and
% Buser~\cite{AlonM84}, and opens up natural conjectures about a potential
% Cheeger and Buser inequality for
% probability density functions supported on manifolds.

Finally, our paper will present a discrete $2$-way clustering algorithm that we
suspect converges to the $(\alpha=1, \gamma=3)$-spectral sweep cut as the
number of data points grows large.  Our
algorithm bears similarity to classic
spectral clustering methods, with some important differences. We note
that we do not prove convergence of this discrete clustering method to
our method for cutting probability densities, and leave this for future work.

% We briefly note some difficulties that we overcome in our work: first,
% graph and manifold Cheeger inequalities do \textit{not} imply Cheeger
% inequalities on Lipschitz density functions. This will be discussed at
% length in Section~\ref{sec:contributions}. In fact, using most
% standard definitions of sparse cuts and eigenfunctions of denstiy
% functions, the Cheeger inequalities are false. Thus, our key
% contribution is not only new mathematical foundations for Cheeger
% inequalities on probability density functions, but also the appropriate
% definitions of quantities like sparse cuts and eigenfunction in this
% setting (which are necessary for the inequalities to hold). For a list of
% mathematical tools necessary to build these inequalities in the
% probability density setting, see Section~\ref{sec:contributions}.

\subsection{Contributions}

Our paper has three core contributions: 
\begin{enumerate}
  \item A natural method for cutting probability density
    functions, based on a new notion of sparse cuts on density functions.
  \item A Cheeger and Buser inequality for probability density
    functions, and
  \item A clustering algorithm operating on samples, which heuristically
    approximates a spectral sweep cut on the density function when the
    number of samples grows large.
\end{enumerate}
We emphasize that our primary contributions are points 1 and 2, which
are formally stated in
Theorems~\ref{thm:sweep-cut} and~\ref{thm:Cheeger-Buser} respectively.  
Our clustering algorithm on samples, which is designed to approximate
the $(\alpha, \gamma)$-spectral sweep cut on the density function as the number of samples
grows large, is of secondary importance. 

We now state our two main theorems. Unfamiliar terms like 
$(\alpha, \beta)$-sparsity, $(\alpha, \gamma)$-spectral sweep cuts, and
$(\alpha,\beta)$-principal eigenvalue are defined in Section~\ref{sec:definitions}.
\begin{theorem} \label{thm:sweep-cut} 
  \textbf{Spectral Sweep Cuts give Sparse Cuts:}

  Let $\rho:\Re^d \to \Re_{\geq 0}$ be an $L$-Lipschitz probability
  density function, and let $\beta = \alpha+1$ and $\gamma = \alpha+2$.
  
  The $(\alpha,\gamma)$-spectral sweep cut of $\rho$ has 
  $(\alpha, \beta)$ sparsity $\Phi$ satisfying:
  \[ 
  \Phi_{OPT} \leq \Phi \leq O(\sqrt{dL\Phi_{OPT}} ).
  \]
  Here, $\Phi_{OPT}$ refers to the optimal $(\alpha,\beta)$ sparsity of
  a cut on $\rho$. 
\end{theorem}

In words, the spectral sweep cut of the
  $(\alpha, \gamma)$  eigenvector gives a provably good approximation to
  the sparsest $(\alpha, \beta)$ cut, as long as $\beta = \alpha+1$ and
  $\gamma = \alpha+2$.  
  Proving this result is a straightforward application of two new
  inequalities we present, which we will refer to as as the Cheeger and Buser inequalities
  for probability density functions.

\begin{theorem}\label{thm:Cheeger-Buser}
  \textbf{Probability Density Cheeger and Buser:}

  Let $\rho:\mathbb{R}^d \rightarrow \mathbb{R \geq 0}$ be an $L$-Lipschitz
  density function. Let $\alpha = \beta - 1 = \gamma - 2$.

  Let $\Phi$ be the infimum $(\alpha,\beta)$-sparsity of a cut through
  $\rho$, and let $\lambda_2$ be the $(\alpha,\gamma)$-principal eigenvalue of
  $\rho$. Then:
  \[ \Phi^2/4 \leq \lambda_2 \]
  and 
  \[\lambda _2 \leq O_{\alpha, \beta}(d \max(L \Phi, \Phi^2)).\]
  The first inequality is \textbf{Probability Density Cheeger}, and
  the second inequality is \textbf{Probability Density Buser}.
\end{theorem}
Note that we don't need $\rho$ to have a total mass of $1$ for any
of our proofs. The overall probability mass of $\rho$ can be arbitrary.

Finally, we give a discrete algorithm~\textsc{1,3-SpectralClutering} for clustering data points into
two-clusters.
We conjecture, but do not prove, that
\textsc{1,3-SpectralClustering} converges to the the $(\alpha=1,
\gamma=3)$-spectral sweep cut of the probability density function $\rho$
as the number of samples grows large.

\begin{algorithm}
  \textsc{1,3-SpectralClustering}

  \textbf{Input:} Point $s_1, \ldots s_n \in \mathbb{R}^d$, and similarity measure
  $K:\mathbb{R}^d, \mathbb{R}^d\rightarrow \mathbb{R}$.
  \begin{enumerate}
    \item Form the affinity matrix $A' \in \mathbb{R}^{n \times n}$,
      where $A'_{ij} = K(s_i, s_j)$ for $i \not= j$ and $A_{ii} = 0$ for
      all $i$.
    \item Define $D$ to be the diagonal matrix whose $(i, i)$ element is
      the sum of $A$'s $i^{th}$. Let $L$ be the Laplacian formed
      from the adjacency matrix $D^{1/2}AD^{1/2}$.
    \item Let $u$ be the principal eigenvector of $L$. Find the value
      $t$ where $t := \argmin_s \Phi_{\{u(v) > t\}}$, where $\Phi_S$ is
      the graph conductance of the cut defined by set $S$.
  \end{enumerate}
  \textbf{Output:} Clusters $G_1 = \{v : u(v) > t\}, G_2 = \{v : u(v)
  \leq t\}$.
\end{algorithm}
We note that this strongly resembles the unnormalized spectral
clustering based on the work of Shi and Malik~\cite{ShiMalik97} and Ng,
Weiss, and Jordan~\cite{NgSpectral01}. The major difference is that we build our
Laplacian from the matrix $D^{1/2}AD^{1/2}$ rather than $A$ (which is
the case for unnormalized spectral
clustering~\cite{von2007tutorial, TrillosVariational15}), or
$D^{-1/2}AD^{-1/2}$ (which is the case for normalized spectral
clustering~\cite{von2007tutorial, TrillosVariational15}).
%%% DEFINITION %%%%
\subsubsection{Definitions}\label{sec:definitions}
In this subsection, we define $(\alpha, \beta)$ sparsity, $(\alpha,
\gamma)$ eigenvalues/Rayleigh quotients, and $(\alpha, \gamma)$ sweep
cuts. 

\vspace{2 mm}
\begin{definition} Let $\rho$ be a probability density function with domain
  $\mathbb{R}^d$, and let $A$ be a
  subset of $\mathbb{R}^d$.

  The \textbf{$(\alpha, \beta)$-sparsity} of the cut defined by $A$ is the
  integral of
  $\rho^\beta$ over the cut, divided by the integral of
  $\rho^\alpha$ on the side of the cut where this integral is
  smaller.

\end{definition}
\vspace{2 mm}

\begin{definition}
The \textbf{$(\alpha, \gamma)$-Rayleigh quotient} of $u$ with
respect to $\rho:\Re^d \to \Re_{\geq 0}$ is:

\[
  R_{\alpha, \gamma}(u) \coloneqq \frac{\int_{\Re^d} \rho^\gamma
  |\nabla u|^2}{\int_{\Re^d} \rho^{\alpha}|u|^2} 
\]

A \textbf{$(\alpha, \gamma)$-principal eigenvalue} of $\rho$ is
$\lambda_2$, where:

\[ \lambda_2 := \inf_{\int \rho^\alpha u = 0} R_{\alpha, \gamma}(u). \]

Define a \textbf{$(\alpha, \gamma)$-principal eigenfunction} of
$\rho$ to be a function $u$ such that $R_{\alpha, \gamma}(u) =
\lambda_2$.
\end{definition}
\vspace{2 mm}

Now we define a sweep cut for a given function with respect to a
a positive valued function supported on $\mathbb{R}^d$:

\vspace{2 mm}
\begin{definition} Let $\alpha, \beta$ be two real numbers, and $\rho$ be
  any function from $\Re^d$ to $\Re_{\geq 0}$.
  Let $u$ be any function from $\Re^d \to \Re$, and let $C_t$ be the cut
  defined by the set $\{s \in \Re^d | u(s) > t\}$. 
  
  The \textbf{sweep-cut} algorithm
  for $u$ with respect to $\rho$ returns the cut $C_t$ of minimum $(\alpha,
  \beta)$ sparsity, where this sparsity is measured with respect to $\rho$.

When $u$ is a $(\alpha, \gamma)$-principal eigenfunction, the sweep cut is called
a \textbf{$(\alpha, \gamma)$-spectral sweep cut} of $\rho$.  
\end{definition}
\subsubsection{Additional Definitions}
A function $\rho: \Re^d \to \Re_{\geq 0}$ is
\textbf{$L$-Lipschitz} if $|\rho(x)-\rho(y)|_2 \leq L|x-y|_2$ for
all $x, y \in \Re^d.$

A function is $\rho:\Re^d \to \Re_{\geq 0}$ is
\textbf{$\alpha$-integrable} if $\int_{\Re^d} \rho^\alpha$ is
well defined and finite. Throughout this paper, we assume $\rho$
is always $\alpha$-integrable.

% \subsection{Do $(\alpha, \beta)$-sparse cuts give meaningful cuts of a
% density function?}
% 
% In this section, we suggest that a $(\alpha, \beta)$ sparse cut captures
% machine learning intuition that two data points drawn from the same side of
% the cut are more similar, and two data points drawn from opposite sides of
% the cut are less similar.
% 
% According to machine learning intuition, the ideal cut of a density
% function should partition it into two pieces of relatively high
% probability mass, while cutting through a low amount of probability
% mass.  
% 
% We note that a $(\alpha=1,\beta=2)$-sparse cut agrees with the machine
% learning intuition that an ideal cut should cut through regions
% of low probability density, while splitting the density function
% into two regions of comparatively large density. Moreover,
% choosing $\beta$ to be $2$ instead of $1$
% biases towards longer cuts through lower density regions,
% which agrees with machine learning intuition and practice. We
% will detail the advantages and disadvantages of a $(1,2)$-sparse cut in
% Section~\ref{sec:changing-beta}.


%These inequalities critically depend on the right notion of $(\alpha, \beta)$-sparsity and the principal $(\alpha, \gamma)$-eigenfunctions, and the right relations between $\alpha, \beta$, and $\gamma$.


% The contributions of our paper can be summed up as follows: first, we define the notion of an $(\alpha, \beta)$-sparse cut for a probability density function, which captures the notion of a cut that separates the density into two pieces of high probability mass while cutting through a region of low probability mass. We will then show that $(1,2)$-sparse cuts satisfy this intuition, and have additional desirable properties in machine learning.  Next, we give a spectral clustering-based algorithm that generates a cut of provably low $(1,2)$-sparsity for all Lipschitz probability density functions, as the number of samples grows large.  To prove this, we will state and prove a Cheeger and Buser inequality on probability density functions, which depends critically on the right notion of $(\alpha, \beta)$-sparsity and principal $(\alpha, \beta)$ eigenvalue.  Finally, we show that classical spectral clustering algorithms (like those of Ng.  et al) generate a cut of bad $(\alpha, \beta)$-sparsity for simple $1$-Lipschitz distributions, for any $\alpha, \beta > 0$.

% We note that our Cheeger and Buser inequalities on density functions lead to a natural new conjecture inspired by common machine learning models: is there a Cheeger and Buser inequality for density functions supported on manifolds?  Modeling data as samples from a probability density on a manifold is one of the most influential models in machine learning, and such a theorem would generalize our inequalities and the existing Cheeger/Buser inequalities on manifolds.
%  More generally, we will present clustering algorithms that converge to cuts of provably low $(\alpha, \alpha+1)$-sparsity on the underlying density.  

% \input{introduction/definitions}
% \input{introduction/theorem}
\input{introduction/past-work}
\input{introduction/contributions}

